Deep Proxy Causal Learning and its Application to Confounded Bandit Policy Evaluation

Proxy causal learning (PCL) is a method for estimating the causal effect of treatments on outcomes in the presence of unobserved confounding, using proxies (structured side information) for the confounder. This is achieved via two-stage regression: in the first stage, we model relations among the treatment and proxies; in the second stage, we use this model to learn the effect of treatment on the outcome, given the context provided by the proxies. PCL guarantees recovery of the true causal effect, subject to identifiability conditions. We propose a novel method for PCL, the deep feature proxy variable method (DFPV), to address the case where the proxies, treatments, and outcomes are high-dimensional and have nonlinear complex relationships, as represented by deep neural network features. We show that DFPV outperforms recent state-of-the-art PCL methods on challenging synthetic benchmarks, including settings involving high dimensional image data. Furthermore, we show that PCL can be applied to off-policy evaluation for the confounded bandit problem, in which DFPV also exhibits competitive performance.

==> heishiro_note/mathmacros.tex <==
\global\long\def\score#1{\mathbf{s}_{#1}}%

\global\long\def\hatscore#1{\hat{\mathbf{s}}_{#1}}%

\global\long\def\barscore#1{\bar{\mathbf{s}}_{#1}}%

\global\long\def\tildescore#1{\tilde{{\bf s}}_{#1}}%

\global\long\def\calX{\mathcal{X}}%

\global\long\def\calD{\mathcal{D}}%

\global\long\def\EE{\mathbb{E}}%

\global\long\def\var{\mathrm{Var}}%
\global\long\def\cov{\mathrm{Cov}}%

\global\long\def\calY{\mathcal{Y}}%
\global\long\def\calF{\mathcal{H}}%

\global\long\def\calZ{\mathcal{Z}}%
\global\long\def\calF{\mathcal{F}}%

\global\long\def\inner#1#2{\left\langle #1,#2\right\rangle }%

\global\long\def\la{\langle}%

\global\long\def\ra{\rangle}%
\global\long\def\mmd#1#2{\mathrm{MMD}(#1,#2)}%

\global\long\def\mmdsq#1#2{\mathrm{MMD}^{2}(#1,#2)}%

\global\long\def\mmdsqhat#1#2{\mathrm{\mathrm{\widehat{\mathrm{\mathrm{MMD}^{2}}}}(#1,#2)}}%

\global\long\def\norm#1{\left\Vert #1\right\Vert }%

\global\long\def\Verts#1{\lVert#1\rVert}%

\global\long\def\bignorm#1{\big\Vert#1\big\Vert}%

\global\long\def\Normal#1#2{\mathcal{N}(#1,#2)}%

\global\long\def\dto{\overset{d}{\to}}%
\global\long\def\pto{\overset{p}{\to}}%

\global\long\def\diag{\mathrm{diag}}%

\global\long\def\Pr{\mathrm{Pr}}%

\global\long\def\bfone{\mathbf{1}}%

\global\long\def\bfzero{\mathbf{0}}%

\global\long\def\iidsim{\overset{\mathrm{i.i.d.}}{\sim}}%

\global\long\def\indsim{\overset{\mathrm{ind.}}{\sim}}%

\global\long\def\calX{\mathcal{X}}%

\global\long\def\calD{\mathcal{D}}%

\global\long\def\EE{\mathbb{E}}%

\global\long\def\var{\mathrm{Var}}%

\global\long\def\cov{\mathrm{Cov}}%

\global\long\def\inner#1#2{\left\langle #1,#2\right\rangle }%

\global\long\def\la{\langle}%

\global\long\def\ra{\rangle}%

\global\long\def\Verts#1{\lVert#1\rVert}%

\global\long\def\bignorm#1{\big\Vert#1\big\Vert}%

\global\long\def\do#1{\mathrm{do}(#1)}%

\global\long\def\given{\vert}%

\global\long\def\biggiven{\big\vert}%

\global\long\def\Biggiven{\Big\vert}%

\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}} 

$
\global\long\def\ind{\mathpalette{\independenT}{\perp}}%
$

